Fool Me Once? Contrasting Textual and Visual Explanations in a Clinical Decision-Support Setting

The growing capabilities of AI models are leading to their wider use, including in safety-critical domains. Explainable AI (XAI) aims to make these models safer to use by making their inference process more transparent. However, current explainability methods are seldom evaluated in the way they are intended to be used: by real-world end users. To address this, we conducted a large-scale user study with 85 healthcare practitioners in the context of human-AI collaborative chest X-ray analysis. We evaluated three types of explanations: visual explanations (saliency maps), natural language explanations, and a combination of both modalities. We specifically examined how different explanation types influence users depending on whether the AI advice and explanations are factually correct. We find that text-based explanations lead to significant over-reliance, which is alleviated by combining them with saliency maps. We also observe that the quality of explanations, that is, how much factually correct information they entail, and how much this aligns with AI correctness, significantly impacts the usefulness of the different explanation types.

==> sections/results_bayar.tex <==

% To investigate our hypotheses regarding the impact of explanations on radiologists' diagnostic accuracy, we employed two mixed-effects regression models. The first general model assessed how task type and label truthfulness influenced Human Accuracy, addressing Hypothesis 1. The second, more task-specific model, added an Explanation Quality term, aiming to elucidate the conditions outlined in Hypotheses 2 through 5. Both models accounted for individual variability among radiologists, capturing both overarching and task-specific factors that contribute to diagnostic decisions.
% \subsection*{Hypotheses}
% % \begin{itemize}
% %   \item[\textbf{H1:}] Providing radiologists with multimodal explanations (labels + natural language explanations + heatmaps) will lead to higher diagnostic accuracy compared to labels alone.
%   % \item[\textbf{H2:}] The quality of explanations (NLE and heatmaps) will directly impact the diagnostic accuracy.
% \begin{itemize}
%   \item[\textbf{H1:}] The presence of explanations will be associated with a difference in diagnostic accuracy compared to labels alone.
%   \item[\textbf{H3:}] There will be a difference in the identification of incorrect model predictions when high rated explanations are provided.
%   \item[\textbf{H4:}] There will be a difference in radiologist decisions, when low-rated explanations are provided.
%   \item[\textbf{H5:}] There will be a difference in human accuracy when low-rated explanations are provided, even when the model is correct.
% \end{itemize}

To explore the potential impact of explanations on participants' human accuracy, we employed a mixed-effects regression model. This model is structured to understand how task type, label truthfulness, and explanation quality influence Human Accuracy, while considering the unique contribution of each participant and image.

The model captures both general and task-specific factors contributing to diagnostic decisions, elucidating how different types of explanations might influence the accuracy of diagnoses.

\subsection*{Research Questions}

We use our mixed effect model to tackle the following questions: 
\begin{itemize}
  \item[\textbf{Q1:}] Will the inclusion of explanations lead to a differential in human accuracy as compared to seeing only label suggestions?
  \item[\textbf{Q2:}] Is there an identifiable difference in participants' capability to detect correct model predictions when they are bundled with high-rated explanations?
  \item[\textbf{Q3:}] Will participants' decisions differ when presented with low-rated explanations?
  \item[\textbf{Q4:}] Conversely how will low-rated explanations affect human accuracy when model's prediction is accurate?
\end{itemize}


\subsection*{Models}
% To evaluate the performance of radiologists, we introduce the "Human Accuracy" metric:
% \begin{equation}
% A = 
% \begin{cases} 
% 1, & \text{if } (GT = 1 \, \text{and} \, (R = \text{"Somewhat Accurate"} \\
%    & \text{or} \, \text{"Accurate"})) \\
% 0, & \text{otherwise}
% \end{cases}
% \end{equation}

% Where:
% \begin{itemize}
%   \item \( GT \) is the ground truth label for the image, either 1 (correct) or 0 (incorrect).
%   \item \( R \) is the radiologist's ranking of the label's accuracy, which can be "Inaccurate," "Somewhat Accurate," or "Accurate."
% \end{itemize}
% This metric enables straightforward evaluation of radiologist performance while considering the ground truth of each image.

\subsection{Mixed-Effects Regression Model for Human Accuracy Across All Tasks}

To account for the general factors affecting participant' human accuracy across all tasks, we applied a mixed-effects logistic regression model:

\begin{equation}
\begin{aligned}
\text{logit}(\text{Human Accuracy}) &= \beta_0 \\
&+ \beta_1(\text{Task Name}) \\
&+ \beta_2(\text{Label Truthfulness}) \\
&+ \beta_3(\text{Explanation Quality}) \\
&+ u_{\text{Radiologist}} \\
&+ u_{\text{Image}}
\end{aligned}
\end{equation}


In this equation:
\begin{itemize}
  \item \textit{Human Accuracy} is a binary metric that evaluates radiologist performance. The metric is 1 when the AI-suggested label (\(L\)) is correct and the radiologist's assessment (\(R\)) is ``Somewhat Agree'' or ``Agree'' or when the AI-suggested label (\(L\)) is incorrect and the radiologist's assessment is "Disagree". Otherwise, it's 0. This allows for a straightforward evaluation of radiologist performance. 
  \item \( \beta_0 \) represents the intercept.
  \item \( \beta_1 \) signifies the fixed effect for Task Name, capturing how different tasks influence diagnostic accuracy.
  \item \( \beta_2 \) accounts for the fixed effect for Label Truthfulness, indicating how the truthfulness of the label affects diagnostic accuracy.
  \item \( \beta_3 \) represents the fixed effect for Explanation Quality, measuring the influence of the quality of explanations annotated by experienced radiologists on diagnostic accuracy.
  \item \( u_{\text{Radiologist}} \) serves as the random effect for individual radiologists, acknowledging their unique characteristics and diagnostic habits.
  \item \( u_{\text{Image}} \) represents the random effect for individual images, considering the inherent variability and unique attributes of each image.
\end{itemize}
  


% By employing this two-step approach, we aimed to understand the general and specific factors influencing radiologists' decision-making in medical imaging tasks.

\subsection{Human accuracy Analysis with Annotated Explanations}

For our study, we employed expert evaluations to rate the quality of explanations using a Likart scale rating from 1-7. We then utilize this metric to observe whether, for correct human decisions, the average explanation quality score is higher.

In terms of individual explanations, the model's output and its impact on the participant's decision can be framed as follows:

\begin{itemize}
    \item Good explanations will convince the user of the model's decision when the model is right.
    \item Good explanations will reveal to the user when the model is wrong.
    \item Bad explanations will mislead the user to trust the model when it's wrong.
    \item Bad explanations will confuse the user to contradict the model when it's right.
\end{itemize}

This classification aids in understanding the underlying dynamics of how different types of explanations might affect the decision-making process of participants.
We used the mixed effect model on the subsets of incorrectly labeled and correctly labeled images to answer these questions.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/flowchart_true.png}
    \caption{Decision-Making Process when the AI's Label is True. This flowchart depicts potential pathways from the moment the AI system produces a true label to the participant's eventual decision. The quality of explanations, as determined by the expert evaluations, can influence the participant's decision, which can be categorized as influenced by either a 'Good Explanation' or 'Bad Explanation'.}
    \label{fig:TrueLabelFlowchart}
\end{figure}



% In this study, we distinguish between 'high-rated' and 'low-rated' explanations based on expert evaluations. These expert ratings serve as an operational definition and are central to our hypotheses (H2 to H5). We then employ a four-quadrant framework to conceptually define 'good' and 'bad' explanations. According to this framework:

% Good Explanations will either lead to correct human choices when the AI model's suggestion is correct or reveal to the user when the AI model's suggestion is incorrect.
% Bad Explanations will either mislead the user into making incorrect choices despite a correct AI suggestion or further confuse them when the AI model's suggestion is in fact incorrect.



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/flowchart_true.png}
%     \caption{Decision-Making Process when the AI's Label is True. This flow chart outlines the potential pathways from the moment the AI system produces a label that is true to the radiologist's ultimate decision. High-rated and low-rated explanations can both lead to the same outcomes, classified as `Good Explanation' or `Bad Explanation' based on whether the radiologist makes a correct or incorrect decision.}
%     \label{fig:TrueLabelFlowchart}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/flowchart_false.png}
    \caption{Decision-Making Process when the AI's Label is False. This flow chart depicts the decision-making flow when the AI system provides a label that is false. Similar to Figure~\ref{fig:TrueLabelFlowchart}, it traces how high-rated and low-rated explanations can affect the radiologist's choice, with outcomes subsequently labeled as `Good Explanation' or `Bad Explanation'.}
    \label{fig:FalseLabelFlowchart}
\end{figure}


\subsection{Parameter Sweep: Radiologists and Number of Images using Model and Synthetic Data}

To determine the optimal sample size for our study, we executed a parameter sweep with synthetic data. Our aim was to detect a +5\% increase in mean human accuracy for Task 3 by introducing an artificial effect. Leveraging our mixed-effects regression model, we derived p-values to assess the significance of this effect for various combinations of participants and images.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figures/param_sweep.png}
\caption{P-values as a function of the number of participants and images.}
\end{figure}

Analysis indicates that a combination of 20 radiologists and 20 images reliably detects the introduced effect, suggesting it as a suitable sample size for similar experimental designs.



% To do:
% - use human accuracy to calculate AUC. Potentially based statistical model around AUC. 
% - Study relationship between quality of explanation and user rating of explanation
\subsection{Pilot Study Results}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mean_accuracy_pilot.png}
    \caption{Mean accuracy by the participant during the pilot study.}
    \label{fig:mean_accuracy}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mean_explanation_rating.png}
    \caption{Mean explanation rating provided by the participant during the pilot study.}
    \label{fig:mean_explanation}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mean_ratings_pilot.png}
    \caption{Overall mean ratings given by the participant in the pilot study.}
    \label{fig:mean_ratings}
\end{figure}


The pilot study, conducted with a single participant, yielded several noteworthy observations:

\begin{itemize}
    \item \textbf{Task Accuracy:} 
    Surprisingly, Task 1, where only a label was provided and no explanation, achieved the highest mean accuracy as shown in Figure \ref{fig:mean_accuracy}. This preliminary observation indicates that explanations might not always enhance diagnostic outcomes. However, due to the limited sample size, further studies are required.

    \item \textbf{Explanation Preferences:} 
    The explanation rating, depicted in Figure \ref{fig:mean_explanation}, showed a preference for a combination of heatmap and Natural Language Explanation (NLE). Conversely, NLE alone was the least preferred. This might indicate an inclination towards multi-modal explanations.

    \item \textbf{Rating Distribution:} 
    A glance at the overall mean ratings in Figure \ref{fig:mean_ratings} revealed a consistent "strongly agree" response. This could either reflect genuine agreement or indicate a potential bias in the participant's responses.
\end{itemize}

Given the constraints of the pilot study, these insights are preliminary. Future research with a larger sample size is recommended to validate these findings.

\subsubsection{Mixed-Effects Regression Model Results for Human Accuracy Across All Tasks}

Our mixed-effects logistic regression model revealed significant effects of task type (\( \beta_1 \), coeff = 0.42, \( p < .05 \))  on human accuracy.


\section{Results}
\subsection{Mixed-Effects Regression Model Results}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.1\linewidth]{figures/plot_humanacc_all.png}
    \caption{Mean human accuracy by Task.}
    \label{fig:mean_task_accuracy}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.1\linewidth]{figures/label1_p.png}
    \caption{Mean Human Accuracy per task for incorrect labels.}
    \label{fig:mean_task_accuracy_label1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.1\linewidth]{figures/label0_p.png}
    \caption{Mean Human Accuracy per task for incorrect labels..}
    \label{fig:mean_task_accuracyLlabel0}
\end{figure}


Our mixed-effects logistic regression model showed a clear link between task type (\( \beta_1 \), coeff = 0.42, \( p < .05 \)) and human accuracy. When we looked at the accuracy across different tasks, we found an improvement when AI labels came with explanations. For Task 2 (NLE), accuracy improved by 6.65\%. For Task 3 (Heatmap), it improved by 6.65\%. But for Task 4 (Both Heatmaps and NLE), the improvement was only 6.35\%.

\subsection{Detailed Results for Tasks with Explanations}

For the specific tasks, we found:

- In Task 2 (Images with Heatmaps), the Explanation Quality (\( \beta_3 \)) had a clear effect (coeff = 0.68, \( p < .05 \)).
- In Task 3 (Images with NLE), \( \beta_3 \) was also important (coeff = 0.73, \( p < .01 \)).
- But in Task 4 (Images with both Heatmaps and NLE), \( \beta_3 \) wasn't significant (coeff = 1.02, \( p = .11 \)).

\subsection{Multi-dimensional Analysis of Explanations}

Looking at explanations from multiple angles, we saw:

- For Research Question Q2, high-quality explanations helped people be more accurate when the model was right. This was true for all explanation types.
- For Research Question Q3, high-quality explanations didn't help identify when the model was wrong.
- For Research Question Q4, low-quality explanations did change how radiologists decided, but not in a good way. These explanations made decisions less consistent.
- For Research Question Q5, even if the model was right, low-quality explanations made people less accurate.



% \subsubsection{Mixed-Effects Regression Model Results for Human Accuracy Across All Tasks}

% Our mixed-effects logistic regression model revealed significant effects of task type (\( \beta_1 \), coeff = 0.42, \( p < .05 \))  on human accuracy.

% We used Human Accuracy as a performance metric for all the tasks. We found that when AI labels are paired with explanations, the performance of the participants improves by 8.65\% for Task 2 (Heatmaps), 5.65\% for Task 3 (NLE) and 2.35\% for Task 4 (Both Heatmaps and NLE). 



% \subsubsection{Task-Specific Mixed-Effects Model Results for Human Accuracy in Tasks with Explanations}

% Our task-specific models provided more nuanced insights. For Task 2 (Images with Heatmaps), the coefficient for Explanation Quality (\( \beta_3 \)) was statistically significant (coeff = 0.68, \( p < .05 \)). Similarly, in Task 3 (Images with NLE), \( \beta_3 \) was significant (coeff = 0.73, \( p < .01 \)).
% In Task 4 (Images with both Heatmaps and NLE), \( \beta_3 \) did not show a statistically significant effect (coeff = 1.02, \( p = .11 \)).

% \subsubsection{Quadrant Analysis for the Impact of Annotated Explanations}

% Our quadrant analysis provides a multidimensional view on the influence of explanation quality, both high-rated and low-rated, on radiologist decision-making. This analysis offers valuable insights into Hypotheses H2 to H5.

% For Hypothesis H2, the analysis robustly supports that high-rated explanations positively impact human accuracy when the models output is correct. This was evident across all explanation types, validating our operational definitions and strengthening the empirical basis for quality explanations.

% Contrastingly, Hypothesis H3, which posited a role for high-rated explanations in identifying incorrect model predictions, did not find empirical backing in our study. This suggests that while high-rated explanations may be beneficial for enhancing diagnostic accuracy, they do not necessarily aid in the identification of errors made by the AI model.

% Regarding Hypothesis H4, our analysis showed that low-rated explanations did influence radiologist decisions, but not in a manner that enhanced accuracy or clarified incorrect model outputs. These low-rated explanations generated greater variability in radiologist decisions, indicating a need for improving the quality of explanations for better  performance.

% Finally, Hypothesis H5 examined whether low-rated explanations could still impact human accuracy when the model prediction is correct. Our data indicates that even with a correct model prediction, low-rated explanations led to decreased human accuracy compared to high-rated ones, emphasizing the critical role of explanation quality in effective decision-making.


\subsection{Summary of Testing and Model Insights}

- Results show mixed evidence for the presented research questions.
- Confirming Research Question Q1: Explanations in Task 2, 3, and 4 enhanced diagnostic accuracy versus just using labels.
- In line with Research Question Q2: High-quality explanations led to better accuracy across Tasks 2, 3, and 4.
- The non-significant outcomes for certain research questions might be due to the small group of 15 radiologists. For example, despite the anticipation in Research Question Q3, high-quality explanations didn't always point out when the model erred.

- The main takeaway: Quality explanations are crucial. This supports Research Questions Q1 and Q2.
- Using both Natural Language Explanations (NLE) and heatmaps typically raised accuracy. Yet, combining them didn’t offer added benefits.
- A significant restriction was the small group size (15 radiologists). Even though our model adjusts for some differences, we need bigger studies for wider application.
- Looking at 'good' vs. 'bad' explanations, our multi-dimensional analysis provides clarity:
    - Good ones not just boost accuracy when the model is spot-on, but might (not always confirmed here) flag model mistakes.
    - Bad ones can steer radiologists astray, independent of the model’s correctness, stressing the urgency to enhance explanation models.




% \subsection*{Determining \( n_{\text{radiologists}} \) and \( n_{\text{images}} \)}
% To establish a robust foundation for our investigation, we simulated synthetic data that mimicked the study design and outcomes. A moderate effect size was introduced, reflecting a realistic assumption (why). Our power analysis concluded that a sample size of 15 radiologists and 20 images would provide sufficient power to detect the effect size, while being resource and time feasible.

% \subsection*{Annotating Explanations with Radiologists}
% To ensure explanation quality, explanations for correctly labeled images were annotated by three experienced radiologists. Annotators scored explanations on accuracy (scale 1-7). Higher inter-annotator agreement was observed for NLEs compared to heatmaps. Explanations were re-ranked into "inaccurate," "somewhat accurate," and "very accurate," forming the basis for analyzing the impact of explanation quality on diagnostic accuracy.

% \subsection{Quadrant Analysis with Annotated Explanations}



% \begin{itemize}
%     \item \textbf{Quadrant 1: Good explanations when the model is right}
%     \begin{itemize}
%         \item [Ex Result]: If explanations are of high quality, we might anticipate seeing higher levels of agreement and human accuracy.
%         \item [Ex:]: Radiologists reached a human accuracy of 82\% in Task 4 (both heatmaps and NLE) when coupled with high-quality explanations (average accuracy score of 6.2), compared to 65\% in Task 1 (no explanation).
%     \end{itemize}
    
%     \item \textbf{Quadrant 2: Good explanations when the model is wrong}
%     \begin{itemize}
%         \item [Ex Result]: High-quality explanations should facilitate radiologists in identifying when the model's diagnosis is incorrect.
%         \item [Ex]: With explanations having an average accuracy score of 5.8, radiologists improved their human accuracy by 14\% in Task 4 compared to Task 1.
%     \end{itemize}
    
%     \item \textbf{Quadrant 3: Bad explanations misleading the user}
%     \begin{itemize}
%         \item [Ex. Result]: Lower-quality explanations might lead radiologists to erroneously agree with incorrect model suggestions.
%         \item [Ex:]: Poor-quality explanations (average accuracy score of 2.5) in Task 2 (heatmaps only) resulted in a 26\% rate of false positives, a rise from 18\% in Task 1 (no explanations).
%     \end{itemize}
    
%     \item \textbf{Quadrant 4: Bad explanations causing confusion}
%     \begin{itemize}
%         \item [Ex Result]: Poor explanations could lead to a decline in human accuracy, even when the model's decision is correct.
%         \item [Ex:]: In Task 3 (NLE only), low-quality explanations (average accuracy score of 3.1) caused a decrease in human accuracy to 60\% when the model was actually correct.
%     \end{itemize}
% \end{itemize}


% Explanations that  correctly led the user to rely on the label -- how much they correlate to a high explanation score. Or the average explanation score for these explanations vs. the average explanation score where the model was right but the user didn't trust the model


